Characterizing Ethereum Upgradable Smart Contracts and Their Security Implications

Upgradeable smart contracts (USCs) have been widely adopted to enable modifying deployed smart contracts. While USCs bring great flexibility to developers, improper usage might introduce new security issues, potentially allowing attackers to hijack USCs and their users. In this paper, we conduct a large-scale measurement study to characterize USCs and their security implications in the wild. We summarize six commonly used USC patterns and develop a tool, USCDetector, to identify USCs without needing source code. Particularly, USCDetector collects various information such as bytecode and transaction information to construct upgrade chains for USCs and disclose potentially vulnerable ones. We evaluate USCDetector using verified smart contracts (i.e., with source code) as ground truth and show that USCDetector can achieve high accuracy with a precision of 96.26%. We then use USCDetector to conduct a large-scale study on Ethereum, covering a total of 60,251,064 smart contracts. USCDetecor constructs 10,218 upgrade chains and discloses multiple real-world USCs with potential security issues.

==> 08_findings.tex <==

In this section, we present the findings of our measurement.

\subsection{Pattern Detection}
Table ~\ref{ta:pattern_group} shows the group number and total number of each pattern that our method detected. We analyzed the groups of Proxy Patterns and found one group OwnableDelegateProxy \cite{ownabledelegateproxy} with a number of 154,6462. We analyzed this group in depth. This group was created by the smart contract {\itshape WyvernProxyRegistry} \cite{opensearegistry}, which is maintained by OpenSea. {\itshape WyvernProxyRegistry} creates an OwnableDelegateProxy contract for each seller on OpenSea. The seller owns this contract, and its address is stored in {\itshape WyvernProxyRegistry}. The Wyvern exchange uses this contract to take action on the seller's behalf. Every OwnableDelegateProxy's logic address points to the same contract {\itshape AuthenticatedProxy} \cite{authenticatedproxy}, which is also an upgradeable proxy contract. In our depiction of the patterns, we excluded such upgradeable smart contracts created by the same contract with a strong operational purpose, i.e., for those that are not created by a smart contract.

\begin{table}[h]
  \caption{The Groups of the All Patterns }
  \label{ta:pattern_group}
  \centering
  \begin{threeparttable}

    \begin{tabular}{c|l|l|l} 

 \toprule
 \toprule
 \rowcolor{gray}

     \multicolumn{1}{c|}{Pattern} & \multicolumn{1}{c|}{Group Count} & \multicolumn{1}{c}{Total Count} \\ \midrule
     
     \multicolumn{1}{c|}{Proxy Pattern } & \multicolumn{1}{c|}{4,964} & \multicolumn{1}{c}{1,866,904} \\ \midrule

     \multicolumn{1}{c|}{Mix Pattern } & \multicolumn{1}{c|}{1,528} & \multicolumn{1}{c}{23,114} \\ \midrule
     
    \multicolumn{1}{c|}{ \makecell[c]{Dara Separation \& \\ Strategy Pattern} } & \multicolumn{1}{c|}{20,609} & \multicolumn{1}{c}{44,017}
         \\ \midrule

    \multicolumn{1}{c|}{Metamorphic Contract } & \multicolumn{1}{c|}{285} & \multicolumn{1}{c}{2,776} \\ \midrule
     
     \multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{8,653} & \multicolumn{1}{c}{1,936,657} \\ 

     \bottomrule
     
    \end{tabular}

  \end{threeparttable}
  \end{table}

\subsection{Pattern Depiction}

After we remove the smart contracts created by a contract, we also remove the smart contracts that are logic contracts of proxy contracts in Proxy Pattern. Then we use these smart contracts to do the depiction. Figure 2 plots the numbers of all patterns deployed.


\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/count.png}
  \caption{ Number of Each Pattern }
\end{figure}


\subsection{Security Issues}

In this section, we display the security issues related to upgrades in three aspects. Note that some issues can be directly exploitable, and some can become serious bugs if the contract admin is not careful or less experienced. Next, we break down our findings into three aspects: issues related to the contract admin, issues related to the logic address to be upgraded, and issues related to old and new versions.

\subsection{Contract admin issues }
\subsubsection{No restrictive checks.} When performing an upgrade, restrictive checks to the contract admin must be implemented to ensure that the upgrade action can not be done by anyone other than the contract admin, otherwise, an upgrade may replace the existing logic address to an arbitrary address by anyone. For instance, in the worst case of the Proxy Pattern and Mix Pattern, if the function setter has no restrictive checks on contract admin, then the proxy contract can be hijacked by changing the logic contract to the one controlled by a malicious user. List 1 presents a simplified version of a Mix Pattern contract that has no restrictive check on contract admin, derived from a real-world DApp LANDProxy. The old logic address is directly overwritten by the new one (Ln.3). 

\begin{lstlisting}[caption=LANDProxy,
morekeywords={contract, function, public, require},
emph={bytes, payable},
    emphstyle=\color{teal}, 
    ]
contract Proxy {
    function upgrade(IApplication newContract, bytes data) public {
        currentContract = newContract;
        newContract.initialize(data);
    }

    function () payable public {
        require(currentContract != 0);
        delegatedFwd(currentContract, msg.data);
  }
}
    
\end{lstlisting}

To perform an upgrade by using Metamorphic Contract, the first step is to call a function that can destroy the Metamorphic Contract by using opcode {\itshape SELFDESTRUCT}, if this function has no restrictive check on contract admin, then the contract can be destroyed by anyone, or can be hijacked by recreating a metamorphic contract with restrictive check after destroy. Listing 2 presents a simplified version of a Metamorphic contract that has no restrictive check. Since none of the Metamorphic Contracts we detected provide a source code, we here present the decompiled code of a real-world Metamorphic Contract. The function used to destroy the contract can be directly called by anyone (Ln.5).

\begin{lstlisting}[caption=Decompiled code of a Metamorphic Contract,
morekeywords={def, is, selfdestruct},
emph={stor0, stor1},
    emphstyle=\color{teal}, 
    ]
def storage:
  stor0 is address at storage 0
  stor1 is address at storage 1

def unknownf2769492(): # the function can destroy the contract
  selfdestruct(stor1)
    
\end{lstlisting}

Through our exploration of the list that detects multiple contract admins, we detect a small number of smart contracts that are missing a restrictive check on contract admin. But we believe there are more smart contracts with such vulnerabilities that just haven't shown up through transactions yet. The Table ~\ref{ta:no_check} gives the number of each pattern on Ethereum. 


\begin{table}[h]
  \caption{Detected Missing Contract Admin Chcek of Each Pattern  }
  \label{ta:no_check}
  \centering
  \begin{threeparttable}
    \setlength{\tabcolsep}{10mm}{

        \begin{tabular}{c|l|l|l} 
            \toprule
            \toprule
            \rowcolor{gray}

         \multicolumn{2}{c|}{Pattern} & \multicolumn{2}{c}{Count} \\ \midrule
         
         \multicolumn{2}{c|}{Proxy Pattern } & \multicolumn{2}{c}{0} \\ \midrule
    
         \multicolumn{2}{c|}{Mix Pattern } & \multicolumn{2}{c}{2} \\ \midrule
         
         \multicolumn{2}{c|}{\makecell[c]{Dara Separation \& \\ Strategy Pattern}} & \multicolumn{2}{c}{2} \\ \midrule
         
        \multicolumn{2}{c|}{Metamorphic Contract } & \multicolumn{2}{c}{7} \\ \midrule
         
         \multicolumn{2}{c|}{Total} & \multicolumn{2}{c}{11} \\ 
    
         \bottomrule
        \end{tabular}

    }
  \end{threeparttable}
  \end{table}

Additionally, we detected 80 Metamorphic Contracts that have been upgraded, among these 80 contracts, we found 4 of them are controlled by the phish accounts. One of the contracts still gets the transactions from the phish account.

\subsubsection{Incorrect restrictive implementation.} In UUPS, the proxy contract has the function setter embedded into the logic contract. By calling the function setter, the storage slot on the proxy contract is updated to a new logic contract. As a result, the logic contract will contain a {\itshape DELEGATECALL} for the function setter. Since users always interact with the proxy contract, and never with the logic contract, nothing prevents a malicious user from sending transactions to the logic contract directly. This does not pose a threat, since any changes to the states of the logic contract do not affect the proxy contract, as the storage of the logic contract is never used in the proxy contract. There is, however, an exception. If the direct call to the logic contract triggers a {\itshape SELFDESTRUCT} operation, then the logic contract will be destroyed, and the proxy will end up delegating all calls to an address without any code. A similar effect can be achieved if the logic contract can be made to delegate into a malicious contract that contains a {\itshape SELFDESTRUCT}, then the logic contract will be destroyed. The root underlying it is because the uninitialized logic contract, the ownership of the logic contract can be taken by initializing it, which may provide the requisite permissions to the function setter, and in turn, access {\itshape DELEGATECALL} operation.



\subsection{Logic address issues}

If an upgradeable smart contract function setter doesn't have any contract address checked for the target logic contract, then an upgrade may replace the existing logic contract with a pointer to an arbitrary address, which could lead to irreversible consequences. For instance, In {\itshape Proxy Pattern}, there is a way to upgrade and put the function setter in a logic contract (i.e. UUPS). In this situation, the contract admin could accidentally set the target logic contract to an Externally Owned Address (EOA), the contract will be locked up and cannot be upgraded forever.

Through the list that detects consecutive upgrades to the same address, and a list that detects that the upgraded address is a non-contract address, we detect a quite number of transactions that reflect the logic address issues. We categorize the transactions into five types below. The table ~\ref{ta:logic_issue} gives the number of each class of number detected on Ethereum.

\begin{itemize}
\item {\textbf{The same address.}} The same upgrade was submitted multiple times, resulting in duplicate upgrades.
\item {\textbf{Empty Contract.}} The new address is a contract, but the contract has no states and functions.
\item {\textbf{External owned address.}} The new address is an externally owned address (EOA).
\item {\textbf{Zero address.}} The new address is zero.
\item {\textbf{Non-upgradeable logic address in UUPS.}} The new address is zero, or an EOA, or doesn't contain a function setter.
\end{itemize}


\begin{table}[h]
\footnotesize
  \caption{Detected Logic Issues  }
  \label{ta:logic_issue}
  \centering
    
        \begin{tabular}{c|l|l|l|l|l} 
            \toprule
            \toprule
            \rowcolor{gray}

         \multicolumn{1}{c|}{Pattern} & \multicolumn{1}{c|}{\makecell[c]{The same \\ address}} & \multicolumn{1}{c|}{\makecell[c]{Zero \\ address}} & \multicolumn{1}{c|}{\makecell[c]{EOA \& \\ Empty \\ Contract}} & \multicolumn{1}{c}{\makecell[c]{Non-upgradeable \\ logic address \\ in UUPS}}\\ \midrule
         
         \multicolumn{1}{c|}{Proxy Pattern } & \multicolumn{1}{c|}{286} & \multicolumn{1}{c|}{22}  & \multicolumn{1}{c|}{71} & \multicolumn{1}{c}{229} \\ \midrule
    
         \multicolumn{1}{c|}{Mix Pattern } & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c}{0} \\ \midrule
         
         \multicolumn{1}{c|}{\makecell[c]{Dara Separation \& \\ Strategy Pattern}} & \multicolumn{1}{c|}{292} & \multicolumn{1}{c|}{266}  & \multicolumn{1}{c|}{92} & \multicolumn{1}{c}{0} \\ \midrule
         
         \multicolumn{1}{c|}{Total} & \multicolumn{1}{c|}{637} & \multicolumn{1}{c|}{290} & \multicolumn{1}{c|}{165} & \multicolumn{1}{c}{229} \\ 
    
         \bottomrule
        \end{tabular}

  \end{table}

Next, we further explore whether upgradeable smart contracts with these issues have corrected their logical addresses. We found there still 37 Proxy Pattern proxies' logic contracts are still EOA accounts, and one proxy has encountered a malicious transaction from a phish account so the proxy's creator has set the logic address to zero, and one proxy's logic address points to a contract which contains no functions nor states. Among these 37 proxies whose logic addresses are EOA accounts, we found the logic addresses of 15 of these proxies are set to phish accounts, 12 of which have transactions, which means delegate calls to the EOA accounts and all these transactions are processed successfully but no state changed in the proxies.



\subsection{Contract version issues} 

In {\itshape Contract Migration}, developers first need to deploy a new version of a smart contract, and then transfer the storage and balance from the old 
version to the new version. After migration, the old version should be deprecated, but if the old version is not self-destructed, users can still be able to interact with it even though it has been migrated to the new version.

{\textbf{Old contract still in use.}} There are several reasons why the smart contract needs to migrate, the most critical reason is that the contract has a vulnerability, and users' assets in this contract are at risk. After migration, to remind users of the new address, the deployer may label the contract as an old contract and make an announcement to inform users of the new address. We've collected the labeled old contracts and their announcements on Etherscan and analyzed announcements. 

{\textbf{Token contracts on the exchanges.}}
If the newly deployed contract is a token-based contract, it is important to collaborate with exchanges during migration to be sure that a new contract will be listed and the previous one will be discarded. 




\subsubsection{Off-chain function setter issues}

The function setter is used to replace the old logic contract address with the new one when performing an upgrade. If the function setter does not introduce permission limits, anyone can change the logic contract address to any target contract address. 

{\textbf{Function setter permission issues}}
The upgrade operation should be left to the owner of the smart contract. If a function setter doesn't have permission validation for the caller (i.e. msg.sender), then an attacker could exploit this vulnerability and modify the logic contract address to his own malicious contract. 


{\textbf{Function setter compatibility check issues}}
If an upgradeable smart contract function setter doesn't have any contract address check for the target logic contract, then an attacker could abuse this security issue to disable the contract. For instance, In {\itshape Proxy Pattern}, there is a way to upgrade and put the function setter in a logic contract. In this situation, the attacker could tamper the target logic contract to an Externally Owned Address (EOA), the contract will be locked up and cannot be upgraded forever.

Compatibility Check includes the following:
\begin{itemize}
\item {\textbf{Lack of contract address check}}
\item {\textbf{Lack of zero contract address check}}
\item {\textbf{Lack of equivalency check for new and current contracts}}
\end{itemize}

{\textbf{Challenge and method.}} 
Though we can get the function selectors from the opcodes we've converted from the bytecodes. But still, it is not easy to detect the off-chain function setter issues on the opcodes level. One reason is the poor readability of opcodes.

To address this problem, we use {\itshape Panoramix} to decompile the bytecode at an address. The {\itshape Panoramix} is an EVM decompiler, which is being integrated into Etherscan for decompiling. All contracts of mainnet have been decompiled and put on the website {\itshape Oko} by the maintainer palkeo, therefore, we can access {\itshape Oko} to obtain the decompiled code of the upgradeable contracts we detected. Since the function setter is essentially a simple operation of a variable assignment, the quality of the decompiled code is sufficient.


